Musings on the HashGraph Protocol: Its Security and Its Limitations

The HashGraph Protocol is a Byzantine fault tolerant atomic broadcast protocol. Its novel use of locally stored metadata allows parties to recover a consistent ordering of their log just by examining their local data, removing the need for a voting protocol. Our paper's first contribution is to present a rewritten proof of security for the HashGraph Protocol that follows the consistency and liveness paradigm used in the atomic broadcast literature. In our second contribution, we show a novel adversarial strategy that stalls the protocol from committing data to the log for an expected exponential number of rounds. This proves tight the exponential upper bound conjectured in the original paper. We believe that our proof of security will make it easier to compare HashGraph with other atomic broadcast protocols and to incorporate its ideas into new constructions. We also believe that our attack might inspire more research into similar attacks for other DAG-based atomic broadcast protocols.

==> event-figure.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{figure}




\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,209); %set diagram left start at 0, and has height of 209

%Shape: Rectangle [id:dp31688818699728316] 
\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 199; blue, 226 }  ,fill opacity=1 ] (480,30) -- (620,30) -- (620,50) -- (480,50) -- cycle ;
%Shape: Rectangle [id:dp10577451733092769] 
\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 199; blue, 226 }  ,fill opacity=1 ] (280,30) -- (420,30) -- (420,50) -- (280,50) -- cycle ;
%Shape: Rectangle [id:dp6935466576015223] 
\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 199; blue, 226 }  ,fill opacity=1 ] (80,30) -- (220,30) -- (220,50) -- (80,50) -- cycle ;
%Shape: Rectangle [id:dp037835659987112136] 
\draw  [draw opacity=0][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (280,50) -- (420,50) -- (420,90) -- (280,90) -- cycle ;
%Shape: Rectangle [id:dp7284386512826456] 
\draw  [draw opacity=0][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (280,90) -- (420,90) -- (420,150) -- (280,150) -- cycle ;
%Straight Lines [id:da04990058586371693] 
\draw    (280,50) -- (420,50) ;
%Straight Lines [id:da9919830193529753] 
\draw    (280,70) -- (420,70) ;
%Straight Lines [id:da4813815004034565] 
\draw    (280,90) -- (420,90) ;
%Straight Lines [id:da8776445819219] 
\draw    (280,110) -- (420,110) ;
%Straight Lines [id:da32635187184696635] 
\draw    (280,130) -- (420,130) ;
%Shape: Rectangle [id:dp9643262334668415] 
\draw   (280,30) -- (420,30) -- (420,150) -- (280,150) -- cycle ;
%Shape: Rectangle [id:dp1648758233577461] 
\draw  [draw opacity=0][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (480,50) -- (620,50) -- (620,90) -- (480,90) -- cycle ;
%Shape: Rectangle [id:dp05962800041065097] 
\draw  [draw opacity=0][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (480,90) -- (620,90) -- (620,150) -- (480,150) -- cycle ;
%Straight Lines [id:da608360036137454] 
\draw    (480,50) -- (620,50) ;
%Straight Lines [id:da904397485475377] 
\draw    (480,70) -- (620,70) ;
%Straight Lines [id:da12665562995523294] 
\draw    (480,90) -- (620,90) ;
%Straight Lines [id:da22941873061382] 
\draw    (480,110) -- (620,110) ;
%Straight Lines [id:da6739211981732325] 
\draw    (480,130) -- (620,130) ;
%Shape: Rectangle [id:dp24515430522842296] 
\draw   (480,30) -- (620,30) -- (620,150) -- (480,150) -- cycle ;
%Shape: Rectangle [id:dp47210227699286744] 
\draw  [draw opacity=0][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (80,50) -- (220,50) -- (220,90) -- (80,90) -- cycle ;
%Shape: Rectangle [id:dp6504320282124437] 
\draw  [draw opacity=0][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (80,90) -- (220,90) -- (220,150) -- (80,150) -- cycle ;
%Straight Lines [id:da8576316232189924] 
\draw    (80,50) -- (220,50) ;
%Straight Lines [id:da8488524815510188] 
\draw    (80,70) -- (220,70) ;
%Straight Lines [id:da4998899839098264] 
\draw    (80,90) -- (220,90) ;
%Shape: Rectangle [id:dp1965838019830266] 
\draw   (80,30) -- (220,30) -- (220,150) -- (80,150) -- cycle ;

% Text Node
\draw (316.5,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{createdBy}};
% Text Node
\draw (319,52) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{selfParent}};
% Text Node
\draw (311,72) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{otherParent}};
% Text Node
\draw (121,162) node [anchor=north west][inner sep=0.75pt]   [align=left] {generic};
% Text Node
\draw (328,162) node [anchor=north west][inner sep=0.75pt]   [align=left] {Swirlds};
% Text Node
\draw (326,92) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{height}};
% Text Node
\draw (331,112) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{TXs}};
% Text Node
\draw (315,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{signature}};
% Text Node
\draw (516.5,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{createdBy}};
% Text Node
\draw (519,52) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{selfParent}};
% Text Node
\draw (511,72) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{otherParents}};
% Text Node
\draw (528,162) node [anchor=north west][inner sep=0.75pt]   [align=left] {HotStuff};
% Text Node
\draw (529,92) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{round}};
% Text Node
\draw (521,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{signature}};
% Text Node
\draw (521,112) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{proposal}};
% Text Node
\draw (111,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{createdBy}};
% Text Node
\draw (111,52) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{selfParent}};
% Text Node
\draw (109,72) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{otherParent}};
% Text Node
\draw (101,102) node [anchor=north west][inner sep=0.75pt]   [align=left] {protocol data};


\end{tikzpicture}


\caption{Example event formats (generic, Swirlds, and HotStuff)}
\end{figure}
